Field-rigid Ising antiferromagnetism with giant spin-flip fields in Van der Waals UOTe

Van der Waals antiferromagnets provide a route to thickness-controlled magnetic order, but few combine high-temperature Ising order with conducting, correlated, and topological electronic structure. Here we show that UOTe realizes this combination. Magnetic susceptibility reveals a strongly anisotropic paramagnetic response, while neutron diffraction establishes c-axis antiferromagnetic order below $T_N \simeq 150$ K with an order-parameter exponent $\beta = 0.14$, close to the two-dimensional Ising value. Torque magnetometry further shows that the ordered state remains well described by a uniaxial antiferromagnet below the high-field transition. Pulsed-field magnetization up to 73 T shows that the ordered state survives to very large fields applied along the c axis before entering a broad metamagnetic regime that begins near 50 T, and remains unsaturated at the highest measured field. Angle-dependent proximity detector oscillator measurements show that the metamagnetic instability is set by the field component along the ordered moment direction, providing direct evidence for Ising-like field rigidity. UOTe therefore establishes a field-rigid Ising antiferromagnet with giant spin-flip fields in a compensated Van der Waals metal, where high-temperature c-axis order, quasi-two-dimensional magnetic criticality, Kondo-associated uranium 5f hybridization, metallic transport, and symmetry-enabled topology coexist in a single material.

==> latexmkrc <==
# ============================================================
# Build external supplement aux file before compiling main text
# ============================================================

add_cus_dep('tex', 'aux', 0, 'makeexternaldocument');

sub makeexternaldocument {
    my ($base_name) = @_;

    my $tex_file = "$base_name.tex";

    if (-e $tex_file) {
        print "Building external document: $tex_file\n";
        return system("latexmk -pdf -interaction=nonstopmode -halt-on-error $tex_file");
    } else {
        print "External document not found: $tex_file\n";
        return 1;
    }
}
